Adaptive Learning with Robust Generalization Guarantees

The traditional notion of generalization---i.e., learning a hypothesis whose empirical error is close to its true error---is surprisingly brittle. As has recently been noted in [DFH+15b], even if several algorithms have this guarantee in isolation, the guarantee need not hold if the algorithms are composed adaptively. In this paper, we study three notions of generalization---increasing in strength---that are robust to postprocessing and amenable to adaptive composition, and examine the relationships between them. We call the weakest such notion Robust Generalization. A second, intermediate, notion is the stability guarantee known as differential privacy. The strongest guarantee we consider we call Perfect Generalization. We prove that every hypothesis class that is PAC learnable is also PAC learnable in a robustly generalizing fashion, with almost the same sample complexity. It was previously known that differentially private algorithms satisfy robust generalization. In this paper, we show that robust generalization is a strictly weaker concept, and that there is a learning task that can be carried out subject to robust generalization guarantees, yet cannot be carried out subject to differential privacy. We also show that perfect generalization is a strictly stronger guarantee than differential privacy, but that, nevertheless, many learning tasks can be carried out subject to the guarantees of perfect generalization.

==> Makefile <==
TOP=main
SRC=main composition learning relation prelims wg open compression reduction intro
FLAGS=tex.flags
BIB=refs

.PHONY : clean
.PHONY : all
.PHONY : ps
.PHONY : long
.PHONY : short
.PHONY : comments

all: $(TOP).pdf $(FLAGS)

ps: $(TOP).ps

long: $(SRC:=.tex) $(BIB).bib clean
	@echo '\\fulltrue \\draftfalse' > ${FLAGS}
	@make

short: $(SRC:=.tex) $(BIB).bib clean
	@echo '\\fullfalse \\draftfalse' > ${FLAGS}
	@make

comments: $(SRC:=.tex) $(BIB).bib clean
	@echo '\\fulltrue \\drafttrue' > ${FLAGS}
	@make

%.pdf: $(SRC:=.tex) $(BIB).bib
	latexmk -pdf $<
	latexmk -c

%.ps : %.tex $(BIB).bib
	latexmk -ps $<
	latexmk -c

clean:
	latexmk -C


==> composition.tex <==
\subsection{Composition Theorems}\label{s.composition}

In this section we show that the class of perfectly generalizing mechanisms is closed under adaptive composition, and that the parameters degrade smoothly as more mechanisms are composed.  Variants of the following results were previously known for differentially private mechanisms; we show they also hold for perfectly generalizing mechanisms. \rc{Citations from DP?}

Theorem \ref{thm.basic} says that the composition of multiple $(\beta, \eps, 0)$-perfectly generalizing mechanisms is also perfectly generalizing, where the $\beta$ and $\eps$ parameters ``add up''.

\begin{theorem}[Basic composition]\label{thm.basic}
Let $\cM_i \colon \cX^n\rightarrow \cR_i$ be $(\beta_i, \eps_i, 0)$-perfectly generalizing for $i=1, \ldots, k$.  The composition $\cM_{[k]} \colon \cX^n \rightarrow \cR_1 \times \cdots \times \cR_k$, defined as $\cM_{[k]}(S) = \left( \cM_1(S), \ldots \cM_k(S) \right)$ is $(\sum_{i=1}^k \beta_i, \sum_{i=1}^k \eps_i)$-perfectly generalizing.
\end{theorem}

%\rc{The result will still hold for with $\delta > 0$, but the proof is more complicated.}

\begin{proof}[\Cref{thm.basic}]
Fix any distribution $\cD$, and for all $i \in [k]$ let $\Sim_i(\cD)$ denote the simulator such that $\cM_i(S) \approx_{\eps, \delta} \Sim_i(\cD)$ with probability $1-\beta_i$ when $S\sim_{i.i.d.}\cD^n$.  Define $\Sim_{[k]}(\cD) = \left( \Sim_1(\cD), \ldots, \Sim_k(\cD) \right)$.  For the remainder of the proof, we will assume that $\cM_i(S) \approx_{\eps, \delta} \Sim_i(\cD)$ for all $i \in [k]$, which will be the case with probability at least $1 - \sum_{i=1}^k \beta_i$ over the choice of the sample.

Fix any $(r_1, \ldots, r_k) \in \cR_1 \times \cdots \times \cR_k$:
\begin{align*}
\Pr[\cM_{[k]}(S) = (r_1, \ldots, r_k)] &= \prod_{i=1}^k \Pr[ \cM_i(S) = r_i] \\
&\leq \prod_{i=1}^k e^{\eps_i} \Pr[ \Sim_i(\cD) = r_i] \\
&= e^{\sum_{i=1}^k \eps_i} \Pr[ \Sim_{[k]}(\cD) = (r_1, \ldots, r_k)] 
\end{align*}
For any $\cO \subseteq \cR_1 \times \cdots \times \cR_k$,
\[ \Pr[\cM_{[k]}(S) \in \cO] = \int_{o \in \cO} \Pr[\cM_{[k]}(S) =o] do \leq \int_{o \in \cO} e^{\sum_{i=1}^k \eps_i} \Pr[\Sim_{[k]}(\cD) =o] do = e^{\sum_{i=1}^k \eps_i} \Pr[\Sim_{[k]}(\cD) \in \cO]. \]
A symmetric argument would show that $\Pr[\Sim_{[k]}(\cD) \in \cO] \leq e^{\sum_{i=1}^k \eps_i} \Pr[\cM_{[k]}(S) \in \cO]$.

The mapping $\Sim_{[k]}(\cD)$ serves as a simulator for $\cM_{[k]}(S)$, so $\cM_{[k]}$ is $(\sum_{i=1}^k \beta_i, \sum_{i=1}^k \eps_i, 0)$-perfectly generalizing.
\end{proof}

Theorem \ref{thm.basic} required that when running $k$ perfectly generalizing mechanisms, the $\eps$ parameter must decay linearly in $k$.  Theorem \ref{thm.advcomp} requires the $\eps$ parameter to decay only as $\sqrt{k}$, at the expense of a small loss in the $\delta$ parameter; relative to Theorem \ref{thm.basic}, this allows for quadratically more mechanisms to be composed with the same generalization guarantee.  Further, the guarantees of Theorem \ref{thm.advcomp} continue to hold even when the mechanisms to be composed can be chosen adaptively.  That is, the $i$th mechanism can chosen based on the outputs of the first $i-1$ mechanisms. 

\begin{theorem}[Advanced composition]\label{thm.advcomp}
Let $\cM_{[k]} \colon \cX^n \rightarrow \cR$ be a mechanism with arbitrary $k$-dimensional range $\cR$ such that the output of $\cM_{[k]}$ can be written as $\cM_{[k]}(S) = (y_1, \ldots, y_k)$, where $y_1 = \cM_1(S)$, $y_2 = \cM_2(S; y_1)$, $\ldots$, $y_k = \cM_k(S; y_1, \ldots, y_{k-1})$ and where each $\cM_i$ is $(\beta, \eps, \delta)$-perfectly generalizing (for all values of parameters $y_1, \ldots, y_k$).  Then $\cM_{[k]}$ is $(k \beta, \eps', k \delta + \delta')$-perfectly generalizing for:
\[ \eps' = \sqrt{2k \ln(1/\delta')} \eps + k \eps (e^{\eps} - 1). \]
\end{theorem}

Before proving Theorem \ref{thm.advcomp}, we present four helpful lemmas.  The first says that for a pair of distributions which are $(\eps, \delta)$-close, one can construct an intermediate distribution which is $(\eps, 0)$-close to the first distribution, and $(0, \delta)$-close to the second.

\begin{lemma}\label{lem.intermediate}
If $Y, Z \in \Delta \cR$ for some abstract range $\cR$ and $Y \approx_{\eps, \delta} Z$, then there exists a $W \in \Delta \cR$ such that $W \approx_{\eps, 0} Z$ and $W \approx_{0, \delta} Y$.
\end{lemma}
\begin{proof}
We will construct such a $W$ from the distributions of $Y$ and $Z$.  For each $r \in \cR$, let $Y(r) = \Pr[Y=r]$ and $Z(r) = \Pr[Z=r]$.  Define sets $S$ and $T$:
\[ S = \{ r \; | \; Y(r) > e^{\eps} Z(r) \} \quad \mbox{ and } \quad T = \{ r \; | \; Z(r) > e^{\eps} Y(r) \}. \]
Also define functions $\alpha,\beta \colon \cR \rightarrow \R$:
\[ \alpha(r) = \min \left\{ e^{\eps}, \frac{\delta + Y(r)}{Z(r)} \right\} \quad \mbox{ and } \quad \beta(r) = \max \left\{ e^{-\eps}, \frac{Y(r) - \delta}{Z(r)} \right\}. \]

Define function $W' \colon \cR \rightarrow \R$ as follows:
\[ W'(r) = \begin{cases} Y(r) & \text{ if } r \notin S \cup T \\ \alpha(r) Z(r) & \text{ if } r \in S \\ \beta(r) Z(r) & \text{ if } r \in T \end{cases}. \]
Although we are not yet guaranteed that $W'(r)$ forms a probability distribution over $\cR$, it does satisfy our other desired properties.  By construction for all $r \in \cR$,
\begin{equation}\label{eq.epsdeltaclose} W'(r) \leq e^{\eps} Z(r), \quad Z(r) \leq e^{\eps} W'(r), \quad \mbox{ and } \quad | Y(r) - W'(r) | \leq \delta. \end{equation}

We will now construct a distribution $W \in \Delta \cR$ from $W'$ by either decreasing the weight assigned to $r \in S$ or increasing the weight assigned to $r \in T$.  Note that such changes will maintain the properties of \eqref{eq.epsdeltaclose}.  Let $A_S = \int_{r \in S} \alpha(r) Z(r) dr$ and $A_T = \int_{r \in T} \beta(r) Z(r) dr$.  Also let $A_{W'} = \int_{r \in \cR} W'(r) dr$.

If $A_{W'} > 1$, we scale down the weight of $r \in S$ and define $W \in \Delta \cR$ as:
\[ \Pr[ W = r] = \begin{cases} W'(r) & \text{ if } r \notin S \\ \left( 1 - \frac{A_{W'} - 1}{A_S} \right) W'(r) & \text{ if } r \in S \end{cases}, \quad \forall r \in \cR. \]
If $A_{W'} < 1$, we similarly scale up the weight of $r \in T$ and define $W \in \Delta \cR$ as:
\[ \Pr[ W = r] = \begin{cases} W'(r) & \text{ if } r \notin T \\ \left( 1 + \frac{1 - A_{W'}}{A_T} \right) W'(r) & \text{ if } r \in T \end{cases}, \quad \forall r \in \cR. \]
Then $W \in \Delta \cR$ and $W \approx_{\eps, 0} Z$ and $W \approx_{0, \delta} Y$.

\end{proof}

The following lemma shows that a product distribution of $(0, \delta)$-close distributions maintains the closeness property.  This allows for the construction of vectors which are $(0, \delta')$-close.

\begin{lemma}\label{lem.triangle}
Let $Y, Z \in \Delta \cR_1$ and $Y', Z' \in \Delta \cR_2$ for arbitrary ranges $\cR_1$ and $\cR_2$ such that $Y$ and $Y'$ are both independent from $Z$ and $Z'$.  Then if $Y \approx_{0, \delta_1} Y'$ and $Z \approx_{0, \delta_2} Z'$, then $(Y, Z) \approx_{0, \delta_1 + \delta_2} (Y', Z')$.
\end{lemma}

\begin{proof}
By our independence assumption, 
\[ (Y, Z) \approx_{0, \delta_1} (Y', Z) \approx_{0, \delta_2} (Y', Z'). \]
Then,
\begin{align*}
& \max_{\cO \subseteq \cR_1 \times \cR_2} \left| \Pr [ (Y,Z) \in \cO] - \Pr [ (Y',Z') \in \cO] \right| \\
&= \max_{\cO \subseteq \cR_1 \times \cR_2} \left| \Pr [ (Y,Z) \in \cO] - \Pr [ (Y',Z) \in \cO] + \Pr [ (Y',Z) \in \cO] - \Pr [ (Y',Z') \in \cO] \right| \\
&\leq \max_{\cO \subseteq \cR_1 \times \cR_2} \left| \Pr [ (Y,Z) \in \cO] - \Pr [ (Y',Z) \in \cO] \right| + \max_{\cO \subseteq \cR_1 \times \cR_2} \left| \Pr [ (Y',Z) \in \cO] - \Pr [ (Y',Z') \in \cO] \right| \\
&\leq \delta_1 + \delta_2
\end{align*}
Thus $(Y, Z) \approx_{0, \delta_1 + \delta_2} (Y', Z')$.

\end{proof}

The next lemma translates the worst-case guarantee of $(\eps, 0)$-closeness into an average case guarantee that is asymptotically smaller than $\eps$.  This lemma can be interpreted as bounding the KL-divergence between two distributions that are $(\eps, 0)$-close.

\begin{lemma}[\cite{DRV10}]\label{lem.kldivergence}
If $Y, Z \in \Delta \cR$ and $Y \approx_{\eps, 0} Z$, then,
\[ \E_{y \sim Y} \left[ \ln \frac{ \Pr[ Y = y]}{ \Pr[Z=y]} \right] \leq \eps (e^{\eps} - 1). \]
\end{lemma}

The final lemma used in the proof of Theorem \ref{thm.advcomp} is Azuma's Inequality, a well-known concentration inequality for random variables that are not independent of each other.

\begin{lemma}[Azuma's Inequality]\label{lem.azuma}
Let $C_1, \ldots, C_k$ be real-valued random variables such that for all $i \in [k]$, $\Pr[ | C_i | \leq \alpha ] = 1$, and for every $(c_1, \ldots, c_{i-1}) \in \Supp(C_1, \ldots, C_{i-1})$, we have,
\[ \E[ C_i \; | \; C_1=c_1, \ldots, C_{i-1}=c_{i-1} ] \leq \beta. \]
Then for every $z>0$,
\[ \Pr \left[ \sum_{i=1}^k C_i > k \beta + z \sqrt{k} \alpha \right] \leq e^{-z^2/2}. \]
\end{lemma}



\begin{proof}[\Cref{thm.advcomp}]
Define the simulator for $\cM_{[k]}$ on distribution $\cD$ to be $\Sim_{[k]}(\cD) = (\Sim_1(\cD), \ldots, \Sim_k(\cD))$, where $\Sim_i$ is the simulator for mechanism $\cM_i$.  Let $S \sim_{i.i.d.} \cD^n$.  Because each $\cM_i$ is $(\beta, \eps, \delta)$-perfectly generalizing for all input parameters $(y_1, \ldots, y_{i-1})$, then with probability at least $1-\beta$ over the choice of $S$, $\cM_i(S; y_1, \ldots, y_{i-1}) \approx_{\eps, \delta} \Sim_i(\cD)$.  Taking a union bound, all $k$ mechanisms will be $(\eps, \delta)$ close to their simulators with probability at least $1- k \beta$.  We will assume this is the case for the remainder of the proof.

By Lemma \ref{lem.intermediate}, there exists $W = (W_1, \ldots, W_k)$ such that each $W_i$ satisfies, 
\[ W_i |_{W_1=y_1, \ldots, W_{i-1}=y_{i-1}}\approx_{0, \delta} \cM_i(S; y_1, \ldots, y_{i-1}) \quad \mbox{ and } W_i |_{W_1=y_1, \ldots, W_{i-1}=y_{i-1}} \approx_{\eps, 0} \Sim_i(\cD) |_{y_1, \ldots, y_{i-1}}, \]
for all $i \in [k]$ and all $y_1, \ldots, y_k$.  By a repeated application of Lemma \ref{lem.triangle}, $\cM_{[k]}(S) \approx_{0, k\delta} W$.  Let $y=(y_1, \ldots, y_k)$ denote an element in the range of $\cM_{[k]}$, and define the set, 
\[ B = \left\{ y \; | \; \Pr[ W = y ] > e^{\eps'} \Pr[ \Sim_{[k]}(\cD) = y ] \right\}, \]
for $\eps' = \sqrt{2k \ln(1/\delta')} \eps + k \eps (e^{\eps} - 1)$.

We will show that $\Pr[W \in B] \leq \delta'$, and thus for every $\cO \subseteq \cR$,
\begin{align*} \Pr[ \cM_{[k]}(S) \in \cO ] &\leq k \delta + \Pr[W \in \cO ] \\
&\leq k \delta + \Pr[W \in B ] + \Pr[ W \in \cO \setminus B ] \\
&\leq k \delta + \delta' + e^{\eps'} \Pr[ \Sim_{[k]}(\cD) \in \cO ].
\end{align*}

It remains to be shown that $\Pr[W \in B] \leq \delta'$.  For any fixed $y=(y_1, \ldots, y_k)$,
\begin{align*} \ln & \left( \frac{ \Pr[ W=y ]}{ \Pr[ \Sim_{[k]}(\cD) = y]} \right) \\
&= \ln \left( \prod_{i=1}^k \frac{ \Pr[ W_i = y_i \; | \; W_1 = y_1, \ldots, W_{i-1} = y_{i-1} ]}{ \Pr[ \Sim_i(\cD) = y_i \; | \; y_1, \ldots, y_{i-1} ]} \right) \\
&= \sum_{i=1}^k \ln \left( \frac{ \Pr[ W_i = y_i \; | \; W_1 = y_1, \ldots, W_{i-1} = y_{i-1} ]}{ \Pr[ \Sim_i(\cD) = y_i \; | \; y_1, \ldots, y_{i-1} ]} \right) \\
&\overset{\text{def}}{=} \sum_{i=1}^k c_i(y_1, \ldots, y_i).
\end{align*}

For each $i \in [k]$, we analyze the random variable $c_i(y_1, \ldots, y_{i-1}, W_i)$ that is conditioned on previous outputs $(y_1, \ldots, y_{i-1})$.   Since $W_i |_{W_1=y_1, \ldots, W_{i-1}=y_{i-1}} \approx_{\eps, 0} \Sim_i(\cD) |_{y_1, \ldots, y_{i-1}}$, then for any fixed $y_i$, $\left| c_i(y_1, \ldots, y_{i-1}, y_i) \right| \leq  \eps$.  By Lemma \ref{lem.kldivergence}, 
\[ \E[c_i(y_1, \ldots, y_{i-1}, W_i)] \leq \eps (e^{\eps} - 1). \]

Finally, we can apply Azuma's Inequality to the random variables $C_i = c_i(y_1, \ldots, y_{i-1}, W_i)$ with $\alpha = \eps$, $\beta = \eps (e^{\eps} - 1)$ and $z = \sqrt{2 \ln (1/\delta')}$ to see that,
\[ \Pr[W \in B] = \Pr \left[ \sum_{i=1}^k > \eps' \right] < e^{-z^2/2} = \delta', \]
for our previous choice of $\eps' = \sqrt{2k \ln(1/\delta')} \eps + k \eps (e^{\eps} - 1)$.

We have shown that for all $\cO \subseteq \cR$, 
\[ \Pr[ \cM_{[k]}(S) \in \cO] \leq k \delta + \delta' + e^{\eps'} \Pr[ \Sim_{[k]}(\cD) \in \cO]. \]
Swapping the roles of $\cM_{[k]}$ and $\Sim_{[k]}$ would yield a symmetric argument that,
\[ \Pr[ \Sim_{[k]}(\cD) \in \cO] \leq k \delta + \delta' + e^{\eps'} \Pr[ \cM_{[k]}(S) \in \cO]. \]
Thus 
\[ \cM_{[k]}(S) \approx_{\eps', k \delta + \delta'} \Sim_{[k]}(\cD). \]
Recalling our failure probability of $k \beta$, $\cM_{[k]}$ is $(k \beta, \eps', k \delta + \delta')$-perfectly generalizing for $\eps' = \sqrt{2k \ln(1/\delta')} \eps + k \eps (e^{\eps} - 1)$.

\end{proof}











==> conjecture.tex <==

\subsection{A Conjecture on Robust Generalizing Learning}

\iffalse The result of~\Cref{thm:compressRG} gives us a novel tool to
design robustly generalizing learners for several hypothesis
classes. For example, we can learn axis aligned rectangles,
half-spaces, and separating polynomials based on the compression
schemes for these hypothesis classes. Notably, these are examples
where neither the domain nor the hypothesis class is finite, which is
a space of learning problems which cannot generally be solved subject
to differential privacy (or bounded description length algorithms).
This leads us to propose the following conjecture: \fi

The result of~\Cref{thm:compressRG} gives us a novel tool to design
robustly generalizing learners for several hypothesis classes. For
example, we can learn axis aligned rectangles, half-spaces, and
separating polynomials based on the compression schemes for these
hypothesis classes. This leads us to propose the following conjecture:

\begin{conjecture}\label{c:mainopen}
Every PAC learnable hypothesis class is also PAC learnable under
robust generalization.
\end{conjecture}

We will first show that any PAC learnable hypothesis class (i.e., any
hypothesis class with polynomial VC-dimension) is learnable with a
guarantee of robust generalization, but not necessarily with a polynomial
sample size.

\begin{theorem}\label{thm:all}
Let $\cH$ be a hypothesis class with VC dimension $d$, and let
$\alpha,\beta, \eps, \delta\in (0,1/2)$. Then there exists a
$(\alpha,\beta)$-accurate PAC learning algorithm for $\cH$ that
satisfies $(\eps, \delta)$-robust generalization with a sample size
of $\tilde O\left(2^{O(d)} \max\left\{\frac{1}{\alpha},
\frac{1}{\eps^2} \right\} \ln\left(\frac{1}{\delta\gamma}\right)
\right)$.
\end{theorem}
\sw{may need to add this pac bound}
\begin{proof}
We rely on a recent result of~\cite{MY15}, which gives a
compression scheme of size $2^{O(d)}$ for any hypothesis class with VC
dimension $d$. By~\Cref{thm:compressRG} and the sample complexity
bound in~\cite{LW86},  there is $(\alpha, \beta)$-accurate
PAC learner that satisfies $(\eps,\delta)$-robust generalization as
long as the sample size satisfies the stated bound.
\end{proof}

Even though the sample complexity bound has an exponential dependence
on the VC dimension, this result gives us a generic robustly
generalizing learner for any learnable class. Previously, such a generic
robustly generalizing learner was only known in the case when either the hypothesis
class or the domain had bounded size; such results derive from a
differentially private algorithm in~\cite{KLNRS08}.

If one could improve the exponential dependence $2^{O(d)}$ in Theorem~\ref{thm:all} to
$\poly(d)$, our conjecture would hold. Our conjecture is also related
to an longstanding conjecture regarding compression bounds and
learnability.

\begin{conjecture}[\cite{LW86, W03}]\label{warmuth}
For any hypothesis class of VC dimension $d$, there is a compression
scheme of size $O(d)$.
\end{conjecture}

Note that subject to Conjecture~\ref{warmuth}, our
Conjecture~\ref{c:mainopen} is true.

\begin{lemma}
Suppose that Conjecture~\ref{warmuth} holds. Then any hypothesis class
that is PAC learnable is also PAC learnable under robust
generalization.
\end{lemma}
Note, however, that it may be possible to resolve our
Conjecture~\ref{c:mainopen} without resolving
Conjecture~\ref{warmuth}. We will have a more in-depth discussion
in~\Cref{sec:open}.



==> otherstuff.tex <==

\section{Learning with Generalization Guarantees}
Now we focus on the setting of learning: there is a target concept $c$
 that is a subset of $\cX$ (or a function from $\cX$ to $\{0,1\}$). A
 learning algorithm takes a sample $S\sim_{i.i.d.} \cD^n$ as input and
 outputs a hypothesis $h\colon \cX \rightarrow \{0,1\}$. The goal of
 the learning algorithm is to output a hypothesis that has
 low \emph{error} with respect to the target concept $c$ and the
 underlying distribution $\cD$, where the error is defined as
\[
 err(h) = \mathbb{E}_{x\sim \cD} (h\oplus c)(x).
\]

First, we define the notion of accuracy, which captures guarantee that
the output hypothesis has low empirical error on the input sample. 

\begin{definition}[$(\alpha, \beta)$-Accuracy]
We say that a learning algorithm $\cM\colon \cX^n \rightarrow 2^\cX$
is $(\alpha, \beta)$-accurate if with probability at least $1
- \beta$, for any input $x$, $\cM(x)$ outputs a hypothesis $h$ such
that
\[
\frac{1}{n} \sum_{i=1}^n (h \oplus c)(x_{i}) \leq \alpha.
\]
\end{definition}

\subsection{Relation to PAC learning}

\todo{Define PAC and PPAC}

We first show that if a problem is PAC learnable, then it is learnable
under weak generalization.  Similarly we show that if a problem is in
PPAC then it is also learnable under differential privacy.

\begin{claim}
WG $ + $ Accuracy $\equiv $ PAC.
\end{claim}

\begin{claim}
DP $ + $ Accuracy (on sample) $\equiv$ PPAC.
\end{claim}

\begin{claim}
Anything pac-learnable is also pac-learnable under SG.
\end{claim}

\todo{These claims need proofs.}

Therefore, the classes of PAC and PPAC learnable problems are also
learnable under WG and DP respectively, so there are algorithms that
satisfy these first two weaker generalization guarantees.

We next explore the cost in terms of sample complexity of moving between WG/DP and PAC/PPAC.  Note that if a PAC algorithm output an hypothesis based on a sample of sufficient size (at least the sample complexity suggested by VC-dimension), then the output hypothesis should have low empirical error on the sample as well.


\rc{Where does the next claim belong?}
\begin{claim}
Can learn points properly under SG with sample complexity $polylog(1/\beta, 1/\gamma)/(\alpha^2\epsilon^2)$ ($\gamma$ is failure probab of learner).  This puts SG between pure and approx DP in terms of sample complexity for this problem!
\end{claim}

%We made the following speculations about the relations between the
%generalization guarantees and PAC learnability:

%\begin{enumerate}
%\item if a problem is PAC learnable, then it should be learnable under the generalization model. 
%\item if a problem is in PPAC then it is also learnable in the weak generalization model.
%\item \kn{need to understand relationship between what is learnable in PAC and under weak generalization (and in particular, whether we have to "pay" in sample complexity).}
%\item Another observation we made is that, if a PAC algorithm output an hypothesis based on a sample of sufficient size (at least the sample complexity suggested by VC-dimension), then the output hypothesis should have low empirical error on the sample as well. \sw{WG $ + $ Accuracy $\equiv $ PAC.}
%\item \sw{observe: DP $ + $ Accuracy (on sample) $\equiv$ PPAC.}
%\end{enumerate}


%In the
%section, we want to explore (learning) algorithms that satisfy the
%strong generalization guarantee.


%\kn{We discussed sample complexity: can learn points properly with SG with sample complexity $polylog(1/\beta, 1/\gamma)/(\alpha^2\epsilon^2)$ ($\gamma$ is failure probab of learner). This puts SG between pure and approx DP in terms of sample complexity for this problem!}

%\kn{can one learn points over real with SG?}

%\kn{anything pac-learnable is also pac-learnable under SG}


\subsection{Relation between SQ Learning and SG Learning}

\todo{Define SQ learning}

We now show that the class of SG learnable problems contain the ones
that are SQ learnable. We also give a SG algorithm for learning parity
functions.

\begin{theorem}
Let $\cC$ be a concept class over $\cX$.Suppose that $\cC$ is SQ
learnable using a hypothesis class $\cH$, then $\cC$ is SQ learnable
using $\cH$ by an SG learner.
\end{theorem}

\begin{proof}
 Suppose we have a SQ learner $\cA$ with access to a SQ-oracle $\cO$
 that answers any statistical query with tolerance $\tau$, and $\cA$
 only queries $\cO$ polynomially many times.  It suffices to show that
 there exists a strong generalizing algorithm that could simulate a
 SQ-oracle (with the same tolerance) only requires polynomial sample
 complexity.

In particular, we could use the Laplace mechanism to simulate the SQ
oracle. Then answering each statistic query would require only
$O(1/\tau^2)$ samples. 
\end{proof}

By the result of~\cite{KLNRS11}, we know that the class of locally
learnable problems is also SG learnable. 

Now consider the following generic learner. Let $\cC$ be a concept
class and $\cH$ be a hypothesis class. Given a sample $T$ of size $n$,
a \emph{generic} learner outputs a random hypothesis in the following
way:
\begin{itemize}
\item for each $h\in \cH$, let $q_h = - h\oplus c$ be the error indicator function, and compute an estimate
$\hat q_h$ for $q(T)$ using the Laplace mechanism
\[
\cA_{G}(T) \colon \mbox{Output hypothesis } h = \arg\max_{h'}  [\hat q_{h'}].
\]
\end{itemize}


\begin{claim}
The generic learner could learn any parity function under polynomial
sample complexity.
\end{claim}

\rc{Relate this claim to SG?}




\section{Limitations of privacy and generalization}

Here are some other results that we suspect are true and might want to prove, including learning tasks that separate the three definitions, and lower bounds.

\begin{enumerate}
\item threshold learning. know how to do WG but don't know how to it under DP
\item propose-test-release might be something we cannot do under SG
\item potential separation: learning point function under SG.  Can a DP point learner be reduced to an SG point learner?
\item lower bound for SG? equivalent packing argument for SG? $\sqrt{n}$-Lower bound for answering a collection of counting queries (variance lower bound for SG); learning point problem: construct a distribution where some mass is on a single point; use the compiler to get some basic lower bounds
\item Theorem \ref{thm.sgtodp} can be used as a tool for translating lowerbounds from DP to lowerbounds to SG. 
\item We know that every SG learner is not DP because it can do something weird on an unlikely database.  This motivates a new definition of $(\epsilon, \delta, \beta)$-DP, which has a distribution over databases, and is $(\epsilon, \delta)$-DP with probability $1-\beta$ over this distribution.
\item does sub-sampling help SG just like it could help with DP? subsampling and aggregate, and take the median
\end{enumerate}




==> sgalgs.tex <==
\section{Strongly generalizing learning algorithms}\label{s.sgalgs}

In this section, we want to explore (learning) algorithms that satisfy
the strong generalization guarantee.  We first introduce some useful
subroutines for learning algorithms.

\subsection{Laplace Mechanism}\label{s.laplace}
Consider the following mechanism that releases an approximate answer
for a query $q\colon \cX\rightarrow [0, 1]$. Given sample
$S\sim_{i.i.d.} \cD^n$, the Laplace mechanism $\cM_b$ releases
\[
\hat q(S) \equiv \frac{1}{n} \sum_{i=1}^n q(S_i) + \nu,
\]
where $\nu$ is random variable drawn from some Laplace distribution
$\Lap\left(b\right)$.

\begin{lemma}
The Laplace mechanism $\cM_b$ is $(\beta, \eps, 0, n)$-strongly
generalizing for $b = \sqrt{\frac{\ln(1/\beta)}{2n\eps^2}}$.
\end{lemma}

\begin{proof}
Let $q(\cD)$ denote $\mathbb{E}_{x\sim \cD} [q(x)]$ and let $q(S)$
denote $\frac{1}{n} \sum_{i=1}^n q(S_i)$, and note that a simulator
has access to $q(\cD)$. By Chernoff-Hoeffding Bound,
\[
\Pr\left[ |n\, q(S) - n\, q(\cD)| > t  \right] \leq \exp(-2t^2/n). 
\]
Then except with probability $\beta$, 
\[
|q(S) - q(\cD)| \leq \sqrt{\frac{\ln(1/\beta)}{2n}}.
\]
Now let $b = \sqrt{\frac{\ln(1/\beta)}{2n\eps^2}}$ and consider
Laplace mechanism $\cM_b$ with the following simulator
$cS\colon \Delta \cX\rightarrow \RR$ such that
\[
\cS(\cD) = q(\cD) + \Lap(b).
\]
By the property of Laplace distribution, we know that
\[
\cM_b(S) \approx_{\eps, 0} \cS(\cD).
\]
This completes the proof.
\end{proof}

\subsection{Report Noisy Max}
%\sw{I think similar idea could show that exponential mechanism is also strongly generalizing with the same $\eps$ and $\alpha$ tradeoff}
Let $q_1, q_2, \ldots, q_m\colon \cX\rightarrow [0,1]$ be a collection
of functions. Given a sample $S\sim_{i.i.d.} \cD^n$, we want to
release the index $j$ of the function with approximately highest
empirical average on $S$, that is $q_j(S) \geq \max_{j'} q_{j'}(S)
- \alpha$.

The \emph{Report Noisy Max} mechanism with parameter $b$ takes a
sample $S$ as input and does the following:
\begin{enumerate}
\item for each $j\in [m]$, let
\[
\hat q_j = q_j(S) + \nu_j,
\]
where $\nu_j\sim \Lap(b)$.

\item release the index $\hat j$ with the highest noisy function value (breaking ties arbitrarily), that is
\[
\hat j = \arg\max_{j\in [m]} \hat q_j.
\]
\end{enumerate}

\begin{lemma}
The report noisy max mechanism with parameter $b
 = \sqrt{\frac{\ln(m/\beta)}{2n\eps^2}}$ is $(\beta, \eps, 0,
 n)$-strongly generalizing.
\end{lemma}

\begin{proof}
By Chernoff-Hoeffding Bound and union bound, we know that with
   probability at least $1 - \beta$,
\[
\max_{j\in [m]} |q_j(S) - q_j(\cD)| \leq \sqrt{\frac{\ln(m/\beta)}{2n}}.
\]
Now set $b = \sqrt{\frac{\ln(m/\beta)}{2n\eps^2}}$, and construct the
following simulator $\cS$:
\begin{itemize}
\item for each $j\in [m]$,
\[
\tilde q_j = q_j(\cD) + \Lap(b)
\]
\item release $\tilde j$ such that
\[
\tilde q_j = \arg\max_{j'\in [m]} \tilde q_{j'}.
\]
\end{itemize}

By the same analysis of~\cite{DR14} of report noisy max, we show that
$\cM(S) \approx_{\eps, 0} \cS(\cD)$.
\end{proof}


